Mirror links have dual odd and generalized Khovanov homology

We show that the generalized Khovanov homology, defined by the second author in the framework of chronological cobordisms, admits a grading by the group $\mathbb{Z}\times\mathbb{Z}_2$, in which all homogeneous summands are isomorphic to the unified Khovanov homology defined over the ring $\mathbb{Z}_{\pi}:=\mathbb{Z}[\pi]/(\pi^2-1)$ (here, setting $\pi$ to $\pm 1$ results either in even or odd Khovanov homology). The generalized homology has $\Bbbk := \mathbb{Z}[X,Y,Z^{\pm 1}]/(X^2=Y^2=1)$ as coefficients, and the above implies that most of automorphisms of $\Bbbk$ fix the isomorphism class of the generalized homology regarded as $\Bbbk$-modules, so that the even and odd Khovanov homology are the only two specializations of the invariant. In particular, switching $X$ with $Y$ induces a derived isomorphism between the generalized Khovanov homology of a link $L$ with its dual version, i.e. the homology of the mirror image $L^!$, and we compute an explicit formula for this map. When specialized to integers it descends to a duality isomorphism for odd Khovanov homology, which was conjectured by A. Shumakovitch.

==> images/pics-tangles.tex <==
\newlength\fntinkwidth
\newlength\fntsize
\newlength\fntshift
\newbox\fntbox

\makeatletter

%% \defPicFonts{family}{name}(x0,y0)(x1,y1):size:<size_factor>[r|c|<empty>|outline_code]{code}

\def\defPicFonts#1#2{\@ifnextchar(%
	{\defPicFonts@getcoords{#1}{#2}}%
	{\defPicFonts@getsize{#1}{#2}(-0.5,-0.5)(0.5,0.5)}}
	
\def\defPicFonts@getcoords#1#2(#3){\@ifnextchar(%
	{\defPicFonts@getsize{#1}{#2}(#3)}%
	{\defPicFonts@getsize{#1}{#2}(0,0)(#3)}}

\def\defPicFonts@getsize#1#2(#3)(#4){\@ifnextchar:%)
	{\defPicFonts@getsizefactor{#1}{#2}{(#3)(#4)}}%
	{\defPicFonts@getsizefactor{#1}{#2}{(#3)(#4)}:W:}}
	
\def\defPicFonts@getsizefactor#1#2#3:#4:{\@ifnextchar<%>
	{\defPicFonts@getoutline{#1}{#2}{#3}{#4}}%
	{\defPicFonts@getoutline{#1}{#2}{#3}{#4}<1>}}

\def\defPicFonts@getoutline#1#2#3#4<#5>{\@ifnextchar[%]
	{\defPicFonts@getcode{#1}{#2}{#3}{#4}{#5}}%
	{\defPicFonts@getcode{#1}{#2}{#3}{#4}{#5}[]}}

\def\defPicFonts@getcode#1#2#3#4#5[#6]#7{%
	\ifx#6r\relax
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{\psframe[linewidth=0.3pt,linestyle=dotted]#3}{#7}%
	\else\ifx#6c\relax
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{\pscircle[linewidth=0.3pt,linestyle=dotted](0,0){0.5}}{#7}%
	\else
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{#6}{#7}%
	\fi\fi
}

%% \defPicFonts@define{family}{name}{coords}{hbox_for_size}{size_factor}{outline_code}{code}
%%
\def\defPicFonts@define#1#2#3#4#5#6#7{%
	%
	%	#1#2 draws the symbol using PS-Tricks unit
	% starred version: with outline
	\expandafter\edef\csname#1#2\endcsname{%
		\noexpand\@ifstar
			{\expandafter\noexpand\csname#1#2@draw\endcsname\noexpand\iftrue\noexpand\fi}%
			{\expandafter\noexpand\csname#1#2@draw\endcsname\noexpand\iffalse\noexpand\fi}}%
	%
	% The drawing macro; ##1 = (\iffalse|\iftrue) and ##2 = \fi determine the presence of the outline
	\expandafter\def\csname#1#2@draw\endcsname##1##2{\begingroup
		\pspicture#3%
			\psset{linewidth=0.5pt,dotsep=1pt,arrowsize=5pt,arrowlength=1}%
			##1#6##2#7%
		\endpspicture\endgroup}%
	%
	% fnt#1#2 draws the symbol as a font
	% starred version: no outline
	\expandafter\edef\csname fnt#2\endcsname{%
		\noexpand\@ifstar
			{\expandafter\noexpand\csname fnt#2@size\endcsname\noexpand\iftrue\noexpand\fi}%
			{\expandafter\noexpand\csname fnt#2@size\endcsname\noexpand\iffalse\noexpand\fi}}%
	%
	% The drawing macro; ##1 = (\iffalse|\iftrue) and ##2 = \fi determine the presence of the outline
	\expandafter\def\csname fnt#2@size\endcsname##1##2{%
		\def\fnt@drawcode{#7##1#6##2}%
		\ifmmode
			\edef\next{\noexpand\mathchoice
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\displaystyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\textstyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\scriptfont\noexpand\scriptstyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\scriptscriptfont\noexpand\scriptscriptstyle}}%
		\else
			\edef\next{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\textstyle}%
		\fi
		\next
	}
	\expandafter\def\csname fnt#2@draw\endcsname##1##2{\begingroup
		\fntinkwidth=\fontdimen8##13\relax
		\setbox\fntbox=\hbox{$\m@th##2#4$}%
		\fntshift= \dp\fntbox	\fntshift=#5\fntshift
		\fntsize = \ht\fntbox	\fntsize=#5\fntsize	\advance\fntsize\fntshift
		\psset{unit=\fntsize,linewidth=\fntinkwidth,dotsep=1pt,arrowsize=7\pslinewidth,arrowlength=0.8,arrowinset=0.6}%
		\hskip\fntinkwidth\ifmmode
			\vcenter{\hbox{\pspicture#3\fnt@drawcode\endpspicture}}%
		\else
			\pspicture[shift=-\fntshift]#3\fnt@drawcode\endpspicture
		\fi\hskip\fntinkwidth
	\endgroup}
}

\makeatother

%%
%%	Crossings and resolutions
%%
\defPicFonts{big}{Circle}:|:{\pscircle[linewidth=0.5pt](0,0.05){0.45}}

\defPicFonts{big}{NWSECr}[r]{%
		\psline(-0.5,-0.5)(0.5,0.5)
		\psline[border=3\pslinewidth](-0.5,0.5)(0.5,-0.5)
}%

\defPicFonts{big}{NESWCr}[r]{%
		\psline(-0.5,0.5)(0.5,-0.5)
		\psline[border=3\pslinewidth](-0.5,-0.5)(0.5,0.5)
}%

\defPicFonts{big}{VertRes}[r]{%
		\psbezier(-0.5,-0.5)(-0.08,0)(-0.08,0)(-0.5,0.5)
		\psbezier( 0.5,-0.5)( 0.08,0)( 0.08,0)( 0.5,0.5)
}%

\defPicFonts{big}{HorRes}[r]{%
		\psbezier(-0.5,-0.5)(0,-0.08)(0,-0.08)(0.5,-0.5)
		\psbezier(-0.5, 0.5)(0, 0.08)(0, 0.08)(0.5, 0.5)
}%

\defPicFonts{big}{HorResCob}[r]{%
		\psbezier(-0.5,-0.5)(0,-0.08)(0,-0.08)(0.5,-0.5)
		\psbezier(-0.5, 0.5)(0, 0.08)(0, 0.08)(0.5, 0.5)
		\psline[linewidth=3\pslinewidth](0,-0.18)(0,0.18)
}%

\defPicFonts{big}{PosCr}[r]{%
		\psline{->}(0.5,-0.5)(-0.55,0.55)
		\psline[border=3\pslinewidth]{->}(-0.5,-0.5)(0.55,0.55)
}%

\defPicFonts{big}{NegCr}[r]{%
		\psline{->}(-0.5,-0.5)(0.55,0.55)
		\psline[border=3\pslinewidth]{->}(0.5,-0.5)(-0.55,0.55)
}%

\defPicFonts{big}{NoCr}[r]{%
		\psbezier{->}(-0.5,-0.5)(-0.08,0)(-0.08,0)(-0.55,0.55)
		\psbezier{->}( 0.5,-0.5)( 0.08,0)( 0.08,0)( 0.55,0.55)
}%

\defPicFonts{big}{PosCrArrowUp}[r]{%
		\psline(0.5,-0.5)(-0.55,0.55)
		\psline[border=5\pslinewidth](-0.5,-0.5)(0.55,0.55)
		\psline[linewidth=0.5\pslinewidth,border=1\pslinewidth]{->}(0,-0.5)(0,0.7)
}%

\defPicFonts{big}{PosCrArrowDown}[r]{%
		\psline(0.5,-0.5)(-0.55,0.55)
		\psline[border=5\pslinewidth](-0.5,-0.5)(0.55,0.55)
		\psline[linewidth=0.5\pslinewidth,border=1\pslinewidth]{<-}(0,-0.7)(0,0.5)
}%

%%
%%	A horizontal full twist tangle
%%
\defPicFonts{tangle}{FullTwist}:|:<1.25>[c]{%
	\psclip{\psframe[linestyle=none](0,-1)(1,1)}
		\psbezier(-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\endpsclip
	\psbezier[border=3\pslinewidth](-0.433,-0.25)(-0.15, 0.33)(0.15, 0.33)(0.433,-0.25)
	\psclip{\psframe[linestyle=none](0.1,-1)(-1,1)}
		\psbezier[border=3\pslinewidth](-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\endpsclip
}

%%
%%	Twisted unknots
%%
\defPicFonts{tangle}{PosTwist}(-1,-0.5)(1,0.5)[r]{%
	\psbezier{C-C}( 0.5,-0.5)( 0.2,-0.5)(-0.2,0.5)(-0.5,0.5)
	\psbezier[border=3\pslinewidth]{C-C}(-0.5,-0.5)(-0.2,-0.5)( 0.2,0.5)( 0.5,0.5)
	\psarc{C-C}(-0.5,0){0.5}{90}{270}%
	\psarc{C-C}(0.5,0){0.5}{-90}{90}%
}

\defPicFonts{tangle}{PosTwistHor}(-1,-0.5)(1,0.5)[r]{\pscustom{%
	\moveto(-0.5,0.5)
	\psarc(-0.5,0){0.5}{90}{270}\curveto(-0.3,-0.5)(-0.2,-0.2)(0,-0.2)\curveto( 0.2,-0.2)( 0.3,-0.5)( 0.5,-0.5)
	\psarc( 0.5,0){0.5}{-90}{90}\curveto( 0.3, 0.5)( 0.2, 0.2)(0, 0.2)\curveto(-0.2, 0.2)(-0.3, 0.5)(-0.5, 0.5)
	\stroke
}}

\defPicFonts{tangle}{PosTwistVert}(-1,-0.5)(1,0.5)[r]{%
	\psarc{C-C}( 0.5,0){0.5}{-90}{90}\psellipticarc{C-C}( 0.5,0)(0.4,0.5){90}{270}%
	\psarc{C-C}(-0.5,0){0.5}{90}{270}\psellipticarc{C-C}(-0.5,0)(0.4,0.5){-90}{90}%
}

%%
%%	First Reidemeister move
%%
\defPicFonts{tangle}{RIline}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.25355, 0.15355)(0, 0.2)(0,0)
	\psbezier(-0.35355,-0.35355)(-0.25355,-0.15355)(0,-0.2)(0,0)
}

\defPicFonts{tangle}{RIx}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.25355, 0.15355)(-0.1,-0.2)(0.1,-0.2)
	\psbezier[border=3\pslinewidth](-0.35355,-0.35355)(-0.25355,-0.15355)(-0.1, 0.2)(0.1, 0.2)
	\psbezier(0.1,0.2)(0.4,0.2)(0.4,-0.2)(0.1,-0.2)
}
	
\defPicFonts{tangle}{RIh}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2, 0)(-0.1, 0.2)(0.1, 0.2)
	\psbezier(0.1,0.2)(0.4,0.2)(0.4,-0.2)(0.1,-0.2)
	\psbezier(-0.35355,-0.35355)(-0.2, 0)(-0.1,-0.2)(0.1,-0.2)
}

\defPicFonts{tangle}{RIv}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2,0)(-0.2,0)(-0.35355,-0.35355)
	\pscircle(0.1,0){0.2}
}

\defPicFonts{tangle}{RIcob}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2,0)(-0.2,0)(-0.35355,-0.35355)
	\pscircle(0.1,0){0.2}
	\psline[linewidth=3\pslinewidth](-0.24,0)(-0.1,0)
}

%%
%%	Second Reidemeister move
%%
\defPicFonts{tangle}{RIIxx}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\psbezier[border=3\pslinewidth](-0.433,-0.25)(-0.15, 0.33)(0.15, 0.33)(0.433,-0.25)
}

\defPicFonts{tangle}{RIIhh}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.3,-0.1)(-0.2, 0.2)(0, 0.2)
	\psbezier(-0.433,-0.25)(-0.3, 0.1)(-0.2,-0.2)(0,-0.2)
	\psbezier(0.433, 0.25)(0.3,-0.1)(0.2, 0.2)(0, 0.2)
	\psbezier(0.433,-0.25)(0.3, 0.1)(0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIhv}:|:<1.25>[c]{%
	\psbezier(0.433,0.25)(0.3,0)(0.3,0)(0.433,-0.25)
	\psarc(0,0){0.2}{-90}{90}
	\psbezier(-0.433, 0.25)(-0.3,-0.1)(-0.2, 0.2)(0, 0.2)
	\psbezier(-0.433,-0.25)(-0.3, 0.1)(-0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIvh}:|:<1.25>[c]{%
	\psbezier(-0.433,0.25)(-0.3,0)(-0.3,0)(-0.433,-0.25)
	\psarc(0,0){0.2}{90}{270}
	\psbezier(0.433, 0.25)(0.3,-0.1)(0.2, 0.2)(0, 0.2)
	\psbezier(0.433,-0.25)(0.3, 0.1)(0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIvv}:|:<1.25>[c]{%
	\psbezier(-0.433,0.25)(-0.3,0)(-0.3,0)(-0.433,-0.25)
	\pscircle(0,0){0.2}
	\psbezier(0.433,0.25)(0.3,0)(0.3,0)(0.433,-0.25)
}

\defPicFonts{tangle}{RIIhhs}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.2,0)(0.2,0)(0.433, 0.25)
	\psbezier(-0.433,-0.25)(-0.2,0)(0.2,0)(0.433,-0.25)
}

%%
%%	Third Reidemeister move
%%
\defPicFonts{tangle}{RIIIax}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(0.35355,0.35355)
	\psline[border=2\pslinewidth](-0.35355,0.35355)(0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIah}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIav}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)(-0.35355, 0.35355)
	\psbezier( 0.35355, 0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIac}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psline[linewidth=5\pslinewidth](0,-0.08839)(0,0.08839)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIahhh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psarc(0,0.2){0.15}{45}{315}
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahhv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\pscircle(0,0.2){0.15}
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psbezier( 0.35355, 0.35355)( 0.2,0.2)( 0.25,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahvh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psarc(0,0.2){0.15}{45}{135}
	\psarc(0,0.2){0.15}{225}{315}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahvv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psbezier( 0.35355, 0.35355)(0.2,0.2)(0.25,0)(0.5,0)
	\psarc(0,0.2){0.15}{-135}{135}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIavhh}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{45}{225}
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIavhv}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{-45}{225}
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psbezier( 0.35355, 0.35355)( 0.2,0.2)( 0.25,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIavvh}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{45}{135}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIavvv}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{-45}{135}
	\psbezier( 0.35355, 0.35355)(0.2,0.2)(0.25,0)(0.5,0)
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIbx}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(0.35355,0.35355)
	\psline[border=2\pslinewidth](-0.35355,0.35355)(0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)(-0.35355, 0.35355)
	\psbezier( 0.35355, 0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbc}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psline[linewidth=5\pslinewidth](0,-0.08839)(0,0.08839)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

%%
%%	Three horizontal lines
%%
\defPicFonts{tangle}{IIIVert}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
}

\defPicFonts{tangle}{IIIVertT}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
	\psline[linewidth=3\pslinewidth](0,0)(0,0.14839)
}

\defPicFonts{tangle}{IIIVertB}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
	\psline[linewidth=3\pslinewidth](0,0)(0,-0.14839)
}

%%
%%	Passing a circle over a link
%%
\defPicFonts{tangle}{CircLeft}(-0.375,-0.5)(0.5,0.5):|:<1.25>[r]{%
	\psline(0.375,-0.5)(0.375,0.5)
	\pscircle(0,0){0.25}
}
\defPicFonts{tangle}{CircRight}(-0.5,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\psline(-0.375,-0.5)(-0.375,0.5)
	\pscircle(0,0){0.25}
}
\defPicFonts{tangle}{CircOver}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\psline(0,-0.5)(0,0.5)
	\pscircle[border=3\pslinewidth](0,0){0.25}
}
\defPicFonts{tangle}{CircUnder}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscircle(0,0){0.25}
	\psline[border=3\pslinewidth](0,-0.5)(0,0.5)
}

\defPicFonts{tangle}{CircOverhh}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscustom{\moveto(0,-0.5)
		\curveto(0,-0.125)(0.25,-0.3)(0.25,0)
		\curveto(0.25,0.15)(0,0.35)(0,0)
		\curveto(0,-0.35)(-0.25,-0.15)(-0.25,0)
		\curveto(-0.25,0.3)(0,0.125)(0,0.5)
		\stroke
	}
}
\defPicFonts{tangle}{CircOverhv}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscustom{\moveto(0,-0.5)\curveto(0,-0.125)(0.25,-0.3)(0.25,0)\curveto(0.25,0.3)(0,0.125)(0,0.5)\stroke}%
	\pscustom{\moveto(0,0)\curveto(0,-0.35)(-0.25,-0.15)(-0.25,0)\curveto(-0.25,0.15)(0,0.35)(0,0)\stroke}%
}
\defPicFonts{tangle}{CircOvervh}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscustom{\moveto(0,-0.5)\curveto(0,-0.125)(-0.25,-0.3)(-0.25,0)\curveto(-0.25,0.3)(0,0.125)(0,0.5)\stroke}%
	\pscustom{\moveto(0,0)\curveto(0,-0.35)(0.25,-0.15)(0.25,0)\curveto(0.25,0.15)(0,0.35)(0,0)\stroke}%
}
\defPicFonts{tangle}{CircOvervv}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscustom{\moveto(0,-0.5)
		\curveto(0,-0.125)(-0.25,-0.3)(-0.25,0)
		\curveto(-0.25,0.15)(0,0.35)(0,0)
		\curveto(0,-0.35)(0.25,-0.15)(0.25,0)
		\curveto(0.25,0.3)(0,0.125)(0,0.5)
		\stroke
	}
}

